Why Do Banks Find Business Process Compliance So Challenging? An Australian Case Study

Banks play an intrinsic role in any modern economy, recycling capital from savers to borrowers. They are heavily regulated and there have been a significant number of well publicized compliance failings in recent years. This is despite Business Process Compliance (BPC) being both a well researched domain in academia and one where significant progress has been made. This study seeks to determine why Australian banks find BPC so challenging. We interviewed 22 senior managers from a range of functions within the four major Australian banks to identify the key challenges. Not every process in every bank is facing the same issues, but in processes where a bank is particularly challenged to meet its compliance requirements, the same themes emerge. The compliance requirement load they bear is excessive, dynamic and complex. Fulfilling these requirements relies on impenetrable spaghetti processes, and the case for sustainable change remains elusive, locking banks into a fail-fix cycle that increases the underlying complexity. This paper proposes a conceptual framework that identifies and aggregates the challenges, and a circuit-breaker approach as an "off ramp" to the fail-fix cycle.

==> tex/archive.tex <==
%Process visibility can highlight the exceptions and help develop a pathway to consolidation in C12.  It can help identify the process design issues and failure points in C10, C13 and C16. It can support both the change management process in C20 and indicate where the automation opportunities are in C16.  Supported by event and case attribute data it can also improve governance line-of-sight by linking operational events to business and risk metrics in C19 and enabling process not system monitoring in C18. It can also help clarify roles and responsibilities in C22. Most importantly it can help fill the gap in knowledge and expertise playing a fundamental role in re-building capability, training and supporting documentation associated with C11 and C17.

%The real issue is that Figure~\ref{fig:data_structure} represents the 1\textsuperscript{st} Order Concepts as orthogonal. In reality, they are inter-related and must be treated holistically. You cannot tackle two or three of the concepts without bumping into issues associated with the rest. This is what creates the underlying complexity that 20 out 22 interviewees referred to. Plus the fact that it is changing rapidly, at scale. This is the real reason why banks find BPC so challenging.

%The question then becomes: how do you address it? The answer lies in why previous attempts have failed and why banks seem to churn their process professionals. The interviewees provide some insight. For example, without changing how the banks think about value, measure process, and attribute process ownership with authority, improvement efforts don't provide the results, in the timeframe required. Executives lose patience and move on to the next thing, or as one interviewee put it: Senior leaders ... want to work on the strategic stuff. I'm not sure processes are seen as strategic enough." Changing this type of culture is not a quick fix.

%At the same time, the pressure to deliver results quickly and the reliance on traditional improvement approaches leads to a focus on the ``happy path" yet exceptions are an integral part of the problem. If the improvement succeeds, the proportion of cases associated with the ``happy path" are so small, the benefits are almost immaterial and do not make a difference to the business results. An additional contributing factor is that the typical process discovery approach is based on a group of SMEs manually mapping out the process. They are time constrained, struggle to access the supporting data and, given the loss of knowledge and experience, focus on the ``happy path" only and can not be relied on to map the process accurately, hence: ``The process is [sic] supposed to happen, is not the process that really happens."

%``So if after a year of starting on this, there's no numbers on the board, other than the expenses associated with this, uh people tend to go off it pretty quickly."

%Hence, without a proven track record and unable to generate a business case that addresses the issues in a sustainable way, the banks are left locked in the same pattern of process failure leading to more controls that make the process more complex and more expensive to automate, hence relying on the heroic efforts of people not to make mistakes, a pattern accelerated by rapid change.%It does not stack up It will take a long time to fix, require significant funding, in an area not perceived by executives to be strategically important and where the value is debatable. Yet as one interviewee questioned do product and process owners actually know their costs? Do they understand the real cost of the exceptions, the real cost of continuing to invest in legacy systems for remediation, the cost of training people on broken processes, the real impact of spaghetti processes on operational risk capital? Answering these questions, once again requires a comprehensive understanding and analysis of existing processes. An analysis of all cases not just those on the ``happy path" wrapped up with heuristics. The second part to this challenge is how to package up bundles of activity that can be aligned to existing programs of work, delivered over short change cycles that demonstrate value in 

%Focusing on these three circuit-breakers will address, at least partially, 18 of the 1\textsuperscript{st} Order Concepts. It's not going to change the nature of the business model, the scale, the types of requirements the disruptive change being introduced by the competition, but ...


%Throughout the transcripts there are references to the lack of end-to-end visibility and the impact it has from impairing root cause analysis, to being able to connect operational data with business and risk data, to being able to follow a process and understand its intent. The most critical requirement from a BPM perspective is to find ways to solve the visibility issue. It is clearly linked to the fragmented nature of a bank's process foundations but a combination of ETL tools and techniques must find ways of stitching together the data to enable Automated Process Discovery - the traditional process discovery techniques do not work. The    

%There are other challenges as the analyst progresses through the BPM lifecycle such as designing preventative controls that do not impede the performance of time-critical processes or the computational complexity of monitoring compliance of tens of thousands of transactions with hundreds of controls in real time.  
%We asked interviewees where would they start if they were in charge of addressing the issues. The majority focused on piggy-backing off existing programs of work. They would select a process that was material to the bank's results, a significant pain-point for executives, with a funded program and senior executive sponsorship already in place. They were adamant it should not be a program in its own right. The objective should be to enable an existing program to deliver better outcomes faster by addressing issues discussed blah, blah non-organizational. 

%The top three issues to address from these findings are: the lack of knowledge and experience; the lack of preventative and proactive controls; and end-to-end visibility. Turning to the last of these first. End-to-end visibility is referenced in many different context from not being able to identify root cause of a problem, to making it easier for operators to understand the downstream consequences of their decisions to not being able to quantify the implications of the exceptions.


% I need to add quotes
%\subsection{Requirements Overload}
%One opportunity is to simplify the requirements load. To do this clearly requires more than a BPM toolkit, but BPM can play a significant role. 

%Throughout the transcripts there are references to a lack of standardization naming conventions, and where there are standards there are ways to get around them. A more rigorous use of taxonomies and ontologies developed in conjunction with the regulators and used as the basis for ongoing regulatory oversight may be a path forward, not least of which is standardising across the four regulators and principal agencies such as AUSTRAC. There are additional benefits for both the banks and the regulators here by relying on data and not samples to monitor compliance. One interviewee shared an example where relevant data for all transactions not just a sample of 50 were shared with a regulator following a process mining exercise which took seven hours to develop and seven minutes to run not the usual two to three months. A standard taxonomy implies the banks know what the regulator is looking for and a reliance on population data mean the banks can demonstrate they are not as disjointed as the regulators believe.

%As the findings make clear, it is not just regulatory requirements that add to the load. Industry codes of practice are also a significant contributor and banks don't always control the end-to-end process for their products, e.g. most payments are dependent on at least two banks~\footnote{The exceptions are where payments are ``on-us", i.e. both sending and receiving accounts are held by the same bank.}

%From a BPC perspective there are a number of standard change management aspects to consider here: ensuring all requirements are captured at the start of the project; ensuing that stakeholders are actively engaged and the requirements are clear and understood. However, the real value comes from helping the industry visualise the requirement complexity problem. The term ``siloed" was referenced frequently in many contexts, and they see requirements in silos. Hence, controls will be designed for regulatory requirements, different controls for codes of practice and customer requirements. However, there is often overlap and duplication between the silos -- one requirement will expect a task to be done in 5 days, whereas another, for a different purpose, will expect it to be done in 3. One interviewee stated: `` I think the more controls you put in place, the higher the risk of any process, because you can add complexity..." But banks lack the tools to both visualise and resolve this problem - the maximum control from the minimum number of controls. People need to see their own perspective, but all perspectives have to be available.  

%Reusable requirements

%Perhaps the most significant reference in this study, is to the lack of understanding and knowledge about the requirements that should be in place. The fragmented nature of the process foundations and siloed mentality result in few people understanding the end-to-end requirements, yet for the most part, the maturity of the process means that the requirements have been built in to processes, they're just not visible. Because process discovery is still largely a manual activity and process modelling expertise is limited, when processes are modelled, they are at such a high-level, focus primarily on the ``happy path'' and of such poor quality that the actual requirements do not reveal themselves. Process mining techniques such as variant analysis could be applied by splitting the logs into those that deliver the expected outcome and those that breached

%\subsection{Process Spaghetti}
%The obvious challenge is how to untangle the spaghetti and design and implement business processes that are both fit for pnurpose and meet executive expectations. Given the many failed attempts in the past, possibly the most urgent requirement is an uplift in process maturity as one interviewee put it: ``Most people ... do not understand the fundamentals of what a process is". To counter this another went on to say BPM should be taught as a ``strategic endeavour".

%The process landscape is clearly challenging. The term complex(ity) is referenced 141 times by 20 out of the 22 interviewees. But a comment such as: ``I think complexity comes from ... the fact that no one knows what's going on", raises an interesting question, is it really complex or just complicated because there's been a significant loss of knowledge and experience?  For an industry with such a long history and mature product suite, there is an argument for the latter, which suggests there are potential solutions to simplify.

%A BPM lifecycle approach would suggest Process Identification, Process Discovery and Process Analysis as the first three steps to develop the ``As-Is". : ``[It's] quite difficult to get the cut through to ... see the forest through the trees." 
%But the traditional approach tends to focus on the happy path and a significant component of the complication comes from the exceptions. One interviewee referenced a process that was assumed to operate at 70\% STP, in reality is was 3\% because they hadn't factored in the exceptions. Hence, traditional process discovery tools are not helpful -- especially when process knowledge is such a gap.

%A further step to simplify are tools and techniques to help visualise the exceptions and shine a pathway to consolidation.

%Many interviewees raise the issue of a lack of systems integration and data connectivity. For most business users, whether this is a systems or a data issue is moot. They just want end-to-end visibility about their process. Tools that can stitch data together without common identifiers would be a great leap forward. Automated Process Discovery, when discussed, was warmly welcomed by most. 




%Putting aside the lack of funding for sustainable change, the lack of process maturity is evident in the poor design. 

%The examples provided highlighted a mismatch between the volume-variety characteristics of a process and the design of the process to implement it. Interviewees see automation as a panacea, but recognise that it's not necessarily appropriate for every process, e.g. mortgage processing. It's not a question of knowing what the end state should be, the issue is, as one interviewee put it: ``We're not very good at imagining what it takes to get to achieve that end state" because  So it's difficult to know where to start
 
%``I think complexity comes from ... the fact that no one knows what's going on"

 

%So many of the issues raised from an inability to ``see".


%While the complexity and extent of the requirements is clear, the majority of the references made by interviewees are related to the complexity of the process infrastructure intended to fulfil them. The processes, along with their supporting systems and data, are disjointed and disparate. They are impenetrable, hard to follow, resource intensive and prone to failure.

%Once again this is consistent with the regulatory findings, specifically the references to legacy technology, complex, manual processes, the inadequacy of the controls, responding to issues in a timely manner. The BPC literature's focus on ``compliance by design"~\cite{Governatori2009Journey,awad2010compliance}, run-time monitoring and violation handling~\cite{maggi2014predictive,Barnawi2016antipattern-based} support the regulators' calls for more proactive controls offer potential solutions. While the literature covers proactive controls, the impact on process performance is not discussed. As the second most referenced concept, further work to address this issue is required.

%What is not covered in the literature is solving for the issue where there is a significant loss of knowledge and expertise - the most referenced concept. The literature assumes that there are domain experts covering both requirements and process, presumably with the right level of skills and expertise supported by documentation that exists, is intelligible and applicable. The literature also assumes process models, event streams or the requisite post-execution data exists as inputs. Both the findings from the regulators and the interviews in this study indicate that this is not necessarily the case. 

%Hashmi et al. reference scale and computational complexity as known challenges~\cite{Hashmi2018AreWeDoneYet}. With millions of transactions per day, the scale in banking is clearly significant. But this is compounded by the level of variation - more than 950 ways to open an account, over 55,000 paths through a lending process, more than 400 steps in a mortgage process. Examples from financial services are used throughout the literature, but the examples are high-level, simplified models of the ``happy path" and bear no similarity with the reality experienced by the industry. They are not patched-up, riddled with workarounds, excessive hand-offs and dead-ends. Interviewees also pointed to areas where workflow had been applied, but only to a part of the end-to-end process, negating the potential benefits. None of the solutions in the literature provide evidence that they can support this level of scale and complexity.

%\subsection{Impaired Governance Line-of-Sight}
%A recurring challenge has been the inability to develop a business case for sustainable change. To address the issue sustainable will take a long time and will be expensive, but to date the four major banks are spending half of their investment budget on risk \& compliance programs - it's unlikely that it will demand more. The two remaining issues are executive, which is beyond the scope of this paper and the benefit case. There are clearly aspects of the benefit case that are difficult to calculate but interviewees pointed out that banks do not necessarily know the cost of their products and processes and certainly do not understand the cost imposed by variation. Fertile ground for process analysis.

%of   leave The main issue here is the perceived value



%The study found that there are both technical and cultural challenges that are impeding good governance. C19 and C21 are the third and fourth most referenced concepts.

%Process visibility (C19) is impaired both by an inability to ``connect the dots" across end-to-end processes, aligning business and risk indicators with process data and what one interviewee referred to as ``process myopia", i.e. seeing process as something that exists within boundaries defined by the organizational structure. It is the third most referenced concept and the lack of end-to-end governance is highlighted by the regulators. There are solutions in the literature to connect process events to operational dashboards~\cite{Maggi2012operational}. This study and those in~\cite{Leitner2010Monitoring,Knuplesch2016Visually} also highlight the importance of process monitoring, a gap highlighted in the interviews, where the focus is on systems, not process monitoring.

%Beyond process visibility, governance is made more challenging by the cultural headwinds. The regulators place a significant focus on flaws in the accountability model. This is very evident in this study's findings (C21 - the fourth most referenced concept): i) lack of clarity between the three lines of defence; ii) confusion over ownership with respect to process components and the end-to-end process; iii) increasing reliance on 3rd parties like lawyers and consultants; and iv) a reluctance to make decisions. It is also influenced by: i) multiple teams participating in the end-to-end process (C10); ii) conflicting objectives (C7); and iii) a lack of understanding of both requirements and process (C18). At an executive level, steps have been taken to address this issue under the BEAR regime, but BEAR doe not focus on process accountability directly and does not link the executive lens with the operational lens. Unsurprisingly, the BPC literature does not tackle these issues, yet it assumes clarity of roles, responsibilities and accountability exists.

%Further cultural headwinds are encountered with the investment process. The interviewees make it clear that the banks know what needs to be done, but developing and gaining support for the business case appears to be elusive. This is perhaps not surprising. Costs and execution risks will be high, the time to execute long and the benefit case uncertain. When the typical CEO's tenure in Australia is about five years~\footnote{\url{https://www.afr.com/chanticleer/the-reasons-behind-high-ceo-turnover-20190527-p51rn6#}}, committing to this type of program is high-risk. Hence, the reliance on ``fail-fix", compounding the underlying issues. This is a difficult issue to untangle, the banks are committing significant investor funds to their Risk \& Compliance programs but the proportion that is spent on remediation, perpetuating the patching and workarounds, relative to developing sustainable solutions is unclear.

%The final point concerns compliance culture. On the one hand, progress appears to have been made. Executives have signed-up to the BEAR regime and they have committed significant funding in both resourcing and remediation projects. On the other hand, there is clearly more work to be done. Without the transparency, these cultural headwinds are harder to see and the issues remain hidden. If there is a reluctance to speak-up or see it as "tick-the-box" exercise the real issues will not be visible. Once again, this was referenced in the regulatory reports but is not discussed in the BPC literature.

%\subsection{Process Mining}\label{sec:pm}
%The primary research question in this study was to identify the BPC challenges banks face. As part of the interview process, however, interviewees were also asked if, and how, they thought process mining may be able to address the challenges discussed. The responses were insightful and will form part of future work. In short, they highlighted the potential for Automated Process Discovery to address some of the knowledge gaps and untangle the process web. They also saw online conformance checking, along with predictive and prescriptive monitoring as techniques that would address regulators concerns around a more proactive control environment. The ability to verify compliance against the population and not just a sample was also seen as a potential benefit. The use of case and event attributes was seen as a potential means to help address some of the organizational issues such as aligning accountability and enhancing decision-making line-of-sight.

==> tex/temp.tex <==
\begin{description}
\item[1.1] \textbf{The business model is complex:} The banking business model is clearly complex. There are a large numbers of products and services offered through multiple channels to a wide-range of customer segments across multiple jurisdictions organised around multiple business units as part of an ecosystem dependent on a plethora of 3rd party stakeholders. It's not just the dimensions of the model but the interconnected web that they form, e.g. competitors as customers, products and processes that cut across business units and segments, and that are largely invisible and intangible. Referenced by 21 out of 22 interviewees and prominent in the regulatory reports this complexity drives a significant number of requirements that are constantly changing. While managing requirements change is referenced as an issue in the literature~\cite{Hashmi2018AreWeDoneYet}, the implications for managing BPC under this level of complexity is not specifically covered.
    
\item[1.2] \textbf{Regulatory pressure is intensifying:} There are multiple references in the transcripts to the changing regulatory dynamic, issuing larger fines, with more regulatory requirements and increasing scrutiny. But the regulatory burden is creating other challenges. At a time when regulators are trying to increase the level of competition the cost of compliance is having the opposite effect, with smaller banks struggling to keep up. The burden of compliance is not just falling on the banks it is being felt directly by customers. Furthermore, the de facto financial crime policing role, the regulators now expect the banks to play has significant implications for how employees perceive customers - are they ``good guys" or ``bad guys"?. One final challenge referenced as part of this 1st Order Concept is the fact that the relationship between the banks and the regulators is perceived not to be collaborative undermining the ability to simplify the overall system.
    
\item[1.3] \textbf{Digital innovation and FinTechs are driving rapid change:} The changing competitive dynamics in the industry are also creating more requirements. The challenge stems from the fact that the new players are not burdened by inflexible technology and are far more agile bringing new offerings and value propositions to market. The neobanks face a lighter regulatory burden and the newer players are avoiding the value pools that require a full ADI~\footnote{Authorised Deposit-Taking Institution} license. This competitive pressure is creating a more rapid demand for change.
    
\item[1.4] \textbf{There are frequent changes to business direction and leadership:} The last of the 1st Order Concepts in the \textit{Excessive Requirements, Constantly Changing} theme, referenced by nine interviewees, is somewhat self-inflicted. It refers to the impact repeated changes of the organizational structure and turnover of leadership have on the level of requirements as well as business decisions such as reducing project budgets in-flight, hiring freezes, etc.

\item[2.1] \textbf{The types of requirement vary widely:} ``Compliance with what?" varies depending on the perspective of the interviewee. For some it is strictly regulatory obligations and requirements and for others it includes, industry codes of practice such as Responsible Lending or SWIFT standards, business policy, contractual obligations and, of course, customer requirements. The ambiguity is exacerbated by the varied consequences of failure from the significant fines regulators can impose to an adverse indicator on an SLA report. 

\item[2.2] \textbf{Requirements are hard to interpret, translate and understand:} The way requirements are written is not always clear. They can be contradictory, written in ambiguous language, subject to both interpretation and translation. The challenge is compounded by the lack of understanding of others' perspectives, e.g., the regulators understanding how regulatory requirements are translated into business policy and the internal compliance teams not understanding enough about the underlying products and processes to determining the practicality and application of policy on process. This is rendered more challenging when the requirements are not known - as highlighted in~\cite{APRA2018CBAPrudential,WBC2020Findings} - or stakeholders requirements are not captured up front, given the complexity of the business model.

\item[2.3] \textbf{There are conflicting business objectives and priorities:} Complexity is added to the requirements by the underlying level of conflict in business objectives and priorities. Interviewees referenced the focus on sales, responsiveness, SLAs and cost efficiencies as higher priorities than quality and compliance. Interviewees also reference the emphasis on meeting the needs of investors first and even the threat of larger fines is not sufficient to change the mindset. There is also conflict between different areas in the bank particularly between the Risk \& Compliance function and the revenue generating business units with the later being tasked with being innovative and the former applying the brakes and eliminating risk. This also extends into areas where different revenue generating units rely on the same process but have different objectives.
\end{description}

The combination of these 1st Order Concepts results in banks being confronted by an excessive number of complex requirements, that are hard to translate into process oriented requirements, subject to constant change. This is confirmed in the regulatory reports~\cite{Hayne2019Royal,APRA2018CBAPrudential,WBC2020Findings}. While the literature proposes a range of solutions to address requirement complexity and requirement change, the solutions tackle specific examples of complexity and change not the combined effects of handling the complexity and change at scale.

\subsection{Process Spaghetti}
The scale, complexity and fluidity of requirements presents a significant challenge, but this is compounded by the inadequacy of the process infrastructure tasked with fulfilling them. The processes and their supporting systems and data are disjointed and disparate~(items 3.x). The processes are hard to follow~(items 4.x), they are resource intensive and prone to failure~(items 5.x). 

\begin{description}

\item[3.1] \textbf{Inflexible, legacy technology is poorly integrated:} Banks were early adopters of technology. Systems were typically built for stability and many persist today, some over 40 years old. A mix of in-house build and others sourced from multiple vendors, they are heavily customised, do not integrate easily, and are hard, slow and expensive to change. 

\item[3.2] \textbf{Connecting and accessing data is hard and the quality is poor:} Given the systems-related issues described above, accessing and connecting data is difficult. While there is no shortage of data, classifying it and accessing it, particularly at the right level of granularity, is not easy and there are also gaps. Without unique identifiers and standards such as naming conventions, data doesn't flow easily between technology assets and processes and stitching it together is expensive and time consuming.   
    
\item[3.3] \textbf{Processes are repeatedly fragmented to fit the organization structure:} Processes are seen as something that occurs within a function, not end-to-end. As the organisational structure changes, the process boundaries also change. Over many years this has led to significant fragmentation with bits of processes dispersed across many teams and limited understanding of how the component parts fit together.

\item[4.1] \textbf{Process documentation, supporting tools and materials are inadequate:} This concept covers a range of references from checklists that are so complicated they are not used, to process models developed by people with no/limited process modeling skills. In many cases supporting documentation is not available, not maintained or only covers the ``happy path", and in other cases process maps are documented for the regulators not for the teams operating the processes or as an overlay not an integral part of the process. Repositories are lacking and documentation is often in different formats. This area also covers tools such as improvement methodologies like Lean and Six Sigma which are also inconsistently and inadequately applied. 
    
\item[4.2] \textbf{There are lots of exceptions:} There are many exceptions and variants across processes driven by a drive to meet specific customer needs to a short-term, lower cost solution to a bigger problem. Exceptions are also introduced based on local considerations, e.g. the degree of latency and staff trying to navigate an easier path through the process.

\item[4.3] \textbf{Processes are broken with layers of Band-Aids and patches applied over years:} Years of under investment and constant tweaks and tinkering have left processes strewn with workarounds, patches, bottlenecks and hand-offs, no clear start- and end-point. Change is also applied on a ``fail-fix" basis, hence when the process fails, fixing quickly is essential and this leads to more patches and workarounds.

\item[4.4] \textbf{Change is not always well executed from getting buy-in to embedding the benefits:} With processes so dispersed and so many stakeholders, getting buy-in and capturing requirements up front is challenging. Communicating the change and understanding the benefits and implications are also seen by interviewees as gaps. Interviewees referenced projects running over budget and then being re-scoped, typically leading to more workarounds.

\item[5.1] \textbf{Transaction volumes are significant:} While the scale varies by process, the high volume of time-critical transactions is frequently referenced, e.g. payments. This introduces a number of challenges, e.g. as very short windows of downtime to introduce change, with systems that operate in batch-mode for overnight, end-of-day processing.

\item[5.2] \texbf{Processes are only partially automated bringing in that manual, human element:} Coupled with significant numbers of transactions, even partially automated processes results in high volume of manual, repetitive tasks. It is complicated by the fact that in some cases a whole step in a process is manual, whereas in other some transactions flow ``straight-through", while others are rejected to a manual, repair queue.

\item[5.3] \textbf{Controls are primarily manual and detective, and do not prevent people making mistakes:} Processes are rarely error-proofed. Most controls are after-the-fact, manual and flawed in design. The lack of preventative controls is attributed to the fact they would slow the process down by multiple interviewees.

\item[5.4] \textbf{There aren’t enough people with the right skills, knowledge & experience:} The most frequently referenced 1st Order Concept covers several people related aspects: i) a loss of knowledge and experience as long-tenured resources leave the industry, ii) the narrowing of skills of staff to focus on discrete tasks, iii) the difficulty in attracting talent to work with legacy technology; iv) the time it takes to train new people; and v) the workload pressure the team face. The greatest focus is on the lack of knowledge and understanding of both process and requirements.

\end{description}

\subsection{Impaired Governance Line-of-Sight}
With significant requirement complexity and a tangled web of processes to fulfil them, the third major challenge for banks is their line-of-sight to oversee and govern process compliance is impaired. There are blind spots impacting decision-making across end-to-end processes~(items 6.x) and cultural headwinds that impede progress~(items 7.x).


\begin{description}
\item[6.1] \textbf{End-to-end visibility is poor with inadequate decision-making metrics and reporting:} There is a lack of visibility and transparency across end-to-end processes. Metrics and reporting do not link business outcomes to process performance and systems events, hence decision-making is challenging.

\item[6.2] \textbf{Systems are monitored, processes aren't:} Business activity monitoring and systems monitoring are referenced by multiple interviewees, but while they may trigger alarms in terms of queue depth and system performance they provide no indication of process performance.

\item[7.1] \textbf{Accountability is far from clear:} Accountability is confused. There are owners for the component parts of a process but they are unwilling to cede control to a process owner. Investment in bolstering risk and compliance support resources has only led to accountability being removed one step further from the source of risk. At the same time there is confusion over roles and responsibilities in the three lines of defence model. With the increased regulatory scrutiny, there has been a propensity to bolster remediation and compliance efforts by engaging more consultants and lawyers, once again, shifting accountability from the source of the risk. 

\item[7.2] \textbf{The investment to fix it is too high and will take too long, it's easier to add FTEs:}  The reason for not progressing the case is typically referenced as: the investment is too high, the time to make the changes too long, the benefits unclear and too far in the future when results are needed now. There are also references to a lack of executive interest in this area as it is not seen as cutting-edge.

\item[7.3] \textbf{Compliance is everyone's responsibility but it's just a tick-the-box exercise:} When asked who is responsible for compliance, ``it's everyone's job" was a common response, with the heightened scrutiny creating a sense of nervousness and urgency. However, throughout the transcripts there are references to BPC being perceived as a toll-gate, a "tick-the-box" exercise and a sense of complacency. Perhaps more concerning is the sense of needing to be seen to do the right thing.

\end{description}



One further point of interest was the number of paradoxes that were highlighted:
\begin{enumerate}
    \item The increased regulatory oversight has made banking harder for customers, with the burden of compliance being transferred via increased levels of documentation and form filling: ``...this sort of myriad of complexity, you know, not only is [is] helping the organisation be compliant, but it's hindering the the satisfaction of the customer onboarding into the organisation".
    \item Given the relative concentration within the industry regulators have tried to increase competition, but the cost of compliance is raising the barriers to entry: `` we will never remain competitive, because we just can't invest the money or the resources".
    \item Remediating legacy applications, products and services, has diverted capital from building new infrastructure and extended the life of the problematic legacy.
    \item Investing in more Risk \& Compliance resources has diverted accountability away from the source of risk: `` all the investment in compliance staff, risk staff, risk procedures risk registers, methods, etc. It's actually moved risk management further away from the people who truly do risk management".
    \item The increased focus from the regulators has created a sense of nervousness that has seen wider engagement of lawyers and consultants, further diminishing the level of accountability: ``...we had the lawyers- consultants, external lawyers like, even for a simple obligation". 
    \item The more checks and controls that are added to a process, the less control there is overall: ``we've had a mistake. We're going to put ... an extra control in. That control can sometimes have the negative impact of what we're trying to do."

\end{enumerate}

